On the Cohomology of Two Stranded Braid Varieties

We compute the cohomologies of two strand braid varieties using the two-form present in cluster structures. We confirm these results with proof using Alexander and Poincar\'e duality. Further, we consider products of braid varieties and their interactions with the cohomologies.

==> Figures/cut_iso_diagram.tex <==
% https://q.uiver.app/#q=WzAsNCxbMCwwLCJYKFxcc2lnbWFeYSlcXHRpbWVzIFgoXFxzaWdtYV5iKSJdLFsxLDAsIlgoXFxzaWdtYV57YStiLTF9KSJdLFswLDEsIlxcUGlfezIsYSsxfV57XFxjaXJjLDF9XFx0aW1lcyBcXFBpX3syLGIrMX1ee1xcY2lyYywxfSJdLFsxLDEsIlxcUGlfezIsYStifV57XFxjaXJjLDF9Il0sWzAsMiwiXFxzaW1lcSIsMCx7Im9mZnNldCI6LTV9XSxbMCwyLCJcXHNpbWVxIiwyLHsib2Zmc2V0Ijo1fV0sWzEsMywiXFxzaW1lcSJdLFswLDFdLFsyLDNdXQ==
\begin{tikzcd}
	{X(\sigma^a)\times X(\sigma^b)} & {X(\sigma^{a+b-1})} \\
	{\Pi_{2,a+1}^{\circ,1}\times \Pi_{2,b+1}^{\circ,1}} & {\Pi_{2,a+b}^{\circ,1}}
	\arrow["\begin{rotate}{90}$\simeq$\end{rotate}", shift left=5, from=1-1, to=2-1]
	\arrow["\begin{rotate}{-90}$\simeq$\end{rotate}"', shift right=5, from=1-1, to=2-1]
	\arrow["\begin{rotate}{-90}$\simeq$\end{rotate}", from=1-2, to=2-2]
	\arrow[from=1-1, to=1-2]
	\arrow[from=2-1, to=2-2]
\end{tikzcd}
